Extending Basic Block Versioning with Typed Object Shapes

Typical JavaScript (JS) programs feature a large number of object property accesses. Hence, fast property reads and writes are crucial for good performance. Unfortunately, many (often redundant) dynamic checks are implied in each property access and the semantic complexity of JS makes it difficult to optimize away these tests through program analysis. We introduce two techniques to effectively eliminate a large proportion of dynamic checks related to object property accesses. Typed shapes enable code specialization based on object property types without potentially complex and expensive analyses. Shape propagation allows the elimination of redundant shape checks in inline caches. These two techniques combine particularly well with Basic Block Versioning (BBV), but should be easily adaptable to tracing Just-In-Time (JIT) compilers and method JITs with type feedback. To assess the effectiveness of the techniques presented, we have implemented them in Higgs, a type-specializing JIT compiler for JS. The techniques are compared to a baseline using polymorphic Inline Caches (PICs), as well as commercial JS implementations. Empirical results show that across the 26 benchmarks tested, these techniques eliminate on average 48% of type tests, reduce code size by 17% and reduce execution time by 25%. On several benchmarks, Higgs performs better than current production JS virtual machines

==> stats/againstsm_decr_sm_baseline.tex <==
-267

==> stats/againstsm_decr_sm_no_inlining.tex <==
44

==> stats/againstsm_incr_sm_baseline.tex <==
267

==> stats/againstsm_incr_sm_no_inlining.tex <==
-44

==> stats/againstsm_max_decr_sm_baseline.tex <==
-1

==> stats/againstsm_max_decr_sm_no_inlining.tex <==
76

==> stats/againstsm_max_sm_no_inlining.tex <==
223

==> stats/againstsm_mean_sm_baseline.tex <==
367

==> stats/againstsm_mean_sm_no_inlining.tex <==
56

==> stats/againstsm_min_sm_baseline.tex <==
101

==> stats/againstsm_min_sm_no_inlining.tex <==
24

==> stats/againstsm_num_above_sm_baseline.tex <==
26

==> stats/againstsm_num_above_sm_no_inlining.tex <==
4

==> stats/againstsm_num_below_sm_baseline.tex <==
0

==> stats/againstsm_num_below_sm_no_inlining.tex <==
22

==> stats/againsttr_decr_truffle_100_warmup_itrs.tex <==
-16

==> stats/againsttr_decr_truffle_10_warmup_itrs.tex <==
-334

==> stats/againsttr_incr_truffle_10_warmup_itrs.tex <==
334

==> stats/againsttr_max_decr_truffle_100_warmup_itrs.tex <==
100

==> stats/againsttr_max_decr_truffle_10_warmup_itrs.tex <==
100

==> stats/againsttr_max_truffle_100_warmup_itrs.tex <==
3891

==> stats/againsttr_max_truffle_10_warmup_itrs.tex <==
6990

==> stats/againsttr_mean_truffle_100_warmup_itrs.tex <==
116

==> stats/againsttr_mean_truffle_10_warmup_itrs.tex <==
434

==> stats/againsttr_min_truffle_100_warmup_itrs.tex <==
0

==> stats/againsttr_min_truffle_10_warmup_itrs.tex <==
0

==> stats/againsttr_num_above_truffle_10_warmup_itrs.tex <==
21

==> stats/againsttr_num_below_truffle_100_warmup_itrs.tex <==
13

==> stats/againsttr_num_below_truffle_10_warmup_itrs.tex <==
5

==> stats/againstv8_decr_v8_baseline.tex <==
-115

==> stats/againstv8_incr_v8_baseline.tex <==
115

==> stats/againstv8_incr_v8_no_inlining.tex <==
-49

==> stats/againstv8_max_decr_v8_baseline.tex <==
44

==> stats/againstv8_max_decr_v8_no_inlining.tex <==
76

==> stats/againstv8_max_v8_no_inlining.tex <==
165

==> stats/againstv8_mean_v8_baseline.tex <==
215

==> stats/againstv8_mean_v8_no_inlining.tex <==
51

==> stats/againstv8_min_v8_baseline.tex <==
56

==> stats/againstv8_min_v8_no_inlining.tex <==
24

==> stats/againstv8_num_above_v8_baseline.tex <==
25

==> stats/againstv8_num_above_v8_no_inlining.tex <==
3

==> stats/againstv8_num_below_v8_baseline.tex <==
1

==> stats/againstv8_num_below_v8_no_inlining.tex <==
23

==> stats/callknown_decr_fast_calls.tex <==
10

==> stats/callknown_incr_fast_calls.tex <==
-10

==> stats/callknown_max_decr_fast_calls.tex <==
100

==> stats/callknown_max_fast_calls.tex <==
100

==> stats/callknown_min_fast_calls.tex <==
0

==> stats/callknown_num_above_fast_calls.tex <==
0

==> stats/callknown_num_below_fast_calls.tex <==
12

==> stats/codesize_decr_maxshapes5.tex <==
12

==> stats/codesize_decr_maxshapesinfty.tex <==
2

==> stats/codesize_incr_maxshapes0.tex <==
-17

==> stats/codesize_incr_maxshapes2.tex <==
-17

==> stats/codesize_incr_maxshapes5.tex <==
-12

==> stats/codesize_incr_maxshapesinfty.tex <==
-2

==> stats/codesize_max_decr_maxshapes0.tex <==
26

==> stats/codesize_max_decr_maxshapes2.tex <==
33

==> stats/codesize_max_decr_maxshapes5.tex <==
33

==> stats/codesize_max_decr_maxshapesinfty.tex <==
31

==> stats/codesize_max_maxshapes0.tex <==
87

==> stats/codesize_max_maxshapes2.tex <==
90

==> stats/codesize_max_maxshapes5.tex <==
162

==> stats/codesize_max_maxshapesinfty.tex <==
185

==> stats/codesize_mean_maxshapes0.tex <==
83

==> stats/codesize_mean_maxshapes2.tex <==
83

==> stats/codesize_mean_maxshapes5.tex <==
88

==> stats/codesize_mean_maxshapesinfty.tex <==
98

==> stats/codesize_min_maxshapes0.tex <==
74

==> stats/codesize_min_maxshapes2.tex <==
67

==> stats/codesize_min_maxshapes5.tex <==
67

==> stats/codesize_min_maxshapesinfty.tex <==
69

==> stats/codesize_num_above_maxshapes0.tex <==
0

==> stats/codesize_num_above_maxshapes2.tex <==
0

==> stats/codesize_num_above_maxshapes5.tex <==
1

==> stats/codesize_num_above_maxshapesinfty.tex <==
13

==> stats/codesize_num_below_maxshapes0.tex <==
26

==> stats/codesize_num_below_maxshapes2.tex <==
26

==> stats/codesize_num_below_maxshapes5.tex <==
25

==> stats/codesize_num_below_maxshapesinfty.tex <==
13

==> stats/comptime_decr_maxshapes0.tex <==
1

==> stats/comptime_decr_maxshapes2.tex <==
-1

==> stats/comptime_decr_maxshapes5.tex <==
-10

==> stats/comptime_decr_maxshapesinfty.tex <==
-20

==> stats/comptime_incr_maxshapes0.tex <==
-1

==> stats/comptime_incr_maxshapes5.tex <==
10

==> stats/comptime_max_decr_maxshapes0.tex <==
3

==> stats/comptime_max_decr_maxshapes2.tex <==
3

==> stats/comptime_max_decr_maxshapes5.tex <==
3

==> stats/comptime_max_decr_maxshapesinfty.tex <==
2

==> stats/comptime_max_maxshapes0.tex <==
101

==> stats/comptime_max_maxshapes2.tex <==
113

==> stats/comptime_max_maxshapes5.tex <==
613

==> stats/comptime_max_maxshapesinfty.tex <==
1157

==> stats/comptime_mean_maxshapes0.tex <==
99

==> stats/comptime_mean_maxshapes2.tex <==
101

==> stats/comptime_mean_maxshapes5.tex <==
110

==> stats/comptime_mean_maxshapesinfty.tex <==
120

==> stats/comptime_min_maxshapes0.tex <==
97

==> stats/comptime_min_maxshapes2.tex <==
97

==> stats/comptime_min_maxshapes5.tex <==
97

==> stats/comptime_min_maxshapesinfty.tex <==
98

==> stats/comptime_num_above_maxshapes0.tex <==
1

==> stats/comptime_num_above_maxshapes2.tex <==
25

==> stats/comptime_num_above_maxshapes5.tex <==
25

==> stats/comptime_num_above_maxshapesinfty.tex <==
25

==> stats/comptime_num_below_maxshapes0.tex <==
22

==> stats/comptime_num_below_maxshapes2.tex <==
1

==> stats/comptime_num_below_maxshapes5.tex <==
1

==> stats/comptime_num_below_maxshapesinfty.tex <==
1

==> stats/exectime_decr_maxshapes5.tex <==
25

==> stats/exectime_decr_maxshapesinfty.tex <==
25

==> stats/exectime_incr_maxshapes0.tex <==
-20

==> stats/exectime_incr_maxshapes2.tex <==
-25

==> stats/exectime_incr_maxshapes5.tex <==
-25

==> stats/exectime_incr_maxshapesinfty.tex <==
-25

==> stats/exectime_max_decr_maxshapes0.tex <==
50

==> stats/exectime_max_decr_maxshapes2.tex <==
75

==> stats/exectime_max_decr_maxshapes5.tex <==
75

==> stats/exectime_max_decr_maxshapesinfty.tex <==
75

==> stats/exectime_max_maxshapes0.tex <==
102

==> stats/exectime_max_maxshapes2.tex <==
101

==> stats/exectime_max_maxshapes5.tex <==
117

==> stats/exectime_max_maxshapesinfty.tex <==
104

==> stats/exectime_mean_maxshapes0.tex <==
80

==> stats/exectime_mean_maxshapes2.tex <==
75

==> stats/exectime_mean_maxshapes5.tex <==
75

==> stats/exectime_mean_maxshapesinfty.tex <==
75

==> stats/exectime_min_maxshapes0.tex <==
50

==> stats/exectime_min_maxshapes2.tex <==
25

==> stats/exectime_min_maxshapes5.tex <==
25

==> stats/exectime_min_maxshapesinfty.tex <==
25

==> stats/exectime_num_above_maxshapes0.tex <==
3

==> stats/exectime_num_above_maxshapes2.tex <==
3

==> stats/exectime_num_above_maxshapes5.tex <==
3

==> stats/exectime_num_above_maxshapesinfty.tex <==
4

==> stats/exectime_num_below_maxshapes0.tex <==
22

==> stats/exectime_num_below_maxshapes2.tex <==
23

==> stats/exectime_num_below_maxshapes5.tex <==
20

==> stats/exectime_num_below_maxshapesinfty.tex <==
20

==> stats/memusage_decr_boyer.tex <==
0.64

==> stats/numflips_decr_all_objects.tex <==
99

==> stats/numflips_decr_global_object.tex <==
98

==> stats/numflips_decr_other_objects.tex <==
99

==> stats/numflips_incr_all_objects.tex <==
-99

==> stats/numflips_incr_global_object.tex <==
-98

==> stats/numflips_incr_other_objects.tex <==
-99

==> stats/numflips_max_decr_all_objects.tex <==
100

==> stats/numflips_max_decr_global_object.tex <==
100

==> stats/numflips_max_decr_other_objects.tex <==
100

==> stats/numflips_max_global_object.tex <==
24

==> stats/numflips_max_other_objects.tex <==
17

==> stats/numflips_mean_all_objects.tex <==
1

==> stats/numflips_mean_global_object.tex <==
2

==> stats/numflips_mean_other_objects.tex <==
1

==> stats/numflips_min_all_objects.tex <==
0

==> stats/numflips_min_global_object.tex <==
0

==> stats/numflips_min_other_objects.tex <==
0

==> stats/numflips_num_above_all_objects.tex <==
0

==> stats/numflips_num_above_global_object.tex <==
0

==> stats/numflips_num_above_other_objects.tex <==
0

==> stats/numflips_num_below_all_objects.tex <==
26

==> stats/numflips_num_below_global_object.tex <==
26

==> stats/numflips_num_below_other_objects.tex <==
26

==> stats/readstowrites_mean.tex <==
11.7

==> stats/shapetests_decr_maxshapes0.tex <==
-17

==> stats/shapetests_decr_maxshapes5.tex <==
47

==> stats/shapetests_decr_maxshapesinfty.tex <==
48

==> stats/shapetests_incr_maxshapes2.tex <==
-45

==> stats/shapetests_incr_maxshapes5.tex <==
-47

==> stats/shapetests_incr_maxshapesinfty.tex <==
-48

==> stats/shapetests_max_decr_maxshapes0.tex <==
-0

==> stats/shapetests_max_decr_maxshapes2.tex <==
100

==> stats/shapetests_max_decr_maxshapes5.tex <==
100

==> stats/shapetests_max_decr_maxshapesinfty.tex <==
100

==> stats/shapetests_max_maxshapes0.tex <==
169

==> stats/shapetests_max_maxshapes2.tex <==
134

==> stats/shapetests_max_maxshapes5.tex <==
109

==> stats/shapetests_max_maxshapesinfty.tex <==
109

==> stats/shapetests_mean_maxshapes0.tex <==
117

==> stats/shapetests_mean_maxshapes2.tex <==
55

==> stats/shapetests_mean_maxshapes5.tex <==
53

==> stats/shapetests_mean_maxshapesinfty.tex <==
52

==> stats/shapetests_min_maxshapes0.tex <==
100

==> stats/shapetests_min_maxshapes2.tex <==
0

==> stats/shapetests_min_maxshapes5.tex <==
0

==> stats/shapetests_min_maxshapesinfty.tex <==
0

==> stats/shapetests_num_above_maxshapes0.tex <==
26

==> stats/shapetests_num_above_maxshapes2.tex <==
3

==> stats/shapetests_num_above_maxshapes5.tex <==
3

==> stats/shapetests_num_above_maxshapesinfty.tex <==
2

==> stats/shapetests_num_below_maxshapes0.tex <==
0

==> stats/shapetests_num_below_maxshapes2.tex <==
23

==> stats/shapetests_num_below_maxshapes5.tex <==
23

==> stats/shapetests_num_below_maxshapesinfty.tex <==
24

==> stats/tagtests_decr_property_reads.tex <==
99

==> stats/tagtests_decr_property_writes.tex <==
93

==> stats/tagtests_incr_property_reads.tex <==
-99

==> stats/tagtests_incr_property_writes.tex <==
-93

==> stats/tagtests_max_decr_property_reads.tex <==
100

==> stats/tagtests_max_decr_property_writes.tex <==
100

==> stats/tagtests_max_property_reads.tex <==
43

==> stats/tagtests_max_property_writes.tex <==
159

==> stats/tagtests_mean_property_reads.tex <==
1

==> stats/tagtests_mean_property_writes.tex <==
7

==> stats/tagtests_min_property_reads.tex <==
0

==> stats/tagtests_min_property_writes.tex <==
0

==> stats/tagtests_num_above_property_reads.tex <==
0

==> stats/tagtests_num_above_property_writes.tex <==
2

==> stats/tagtests_num_below_property_reads.tex <==
26

==> stats/tagtests_num_below_property_writes.tex <==
24

==> stats/testcounts_decr_maxshapes0.tex <==
47

==> stats/testcounts_decr_maxshapes5.tex <==
48

==> stats/testcounts_decr_maxshapesinfty.tex <==
49

==> stats/testcounts_incr_maxshapes0.tex <==
-47

==> stats/testcounts_incr_maxshapes2.tex <==
-48

==> stats/testcounts_incr_maxshapes5.tex <==
-48

==> stats/testcounts_incr_maxshapesinfty.tex <==
-49

==> stats/testcounts_max_decr_maxshapes0.tex <==
100

==> stats/testcounts_max_decr_maxshapes2.tex <==
100

==> stats/testcounts_max_decr_maxshapes5.tex <==
100

==> stats/testcounts_max_decr_maxshapesinfty.tex <==
100

==> stats/testcounts_max_maxshapes0.tex <==
100

==> stats/testcounts_max_maxshapes2.tex <==
100

==> stats/testcounts_max_maxshapes5.tex <==
100

==> stats/testcounts_max_maxshapesinfty.tex <==
100

==> stats/testcounts_mean_maxshapes0.tex <==
53

==> stats/testcounts_mean_maxshapes2.tex <==
52

==> stats/testcounts_mean_maxshapes5.tex <==
52

==> stats/testcounts_mean_maxshapesinfty.tex <==
51

==> stats/testcounts_min_maxshapes0.tex <==
0

==> stats/testcounts_min_maxshapes2.tex <==
0

==> stats/testcounts_min_maxshapes5.tex <==
0

==> stats/testcounts_min_maxshapesinfty.tex <==
0

==> stats/testcounts_num_above_maxshapes0.tex <==
0

==> stats/testcounts_num_above_maxshapes2.tex <==
0

==> stats/testcounts_num_above_maxshapes5.tex <==
0

==> stats/testcounts_num_above_maxshapesinfty.tex <==
0

==> stats/testcounts_num_below_maxshapes0.tex <==
26

==> stats/testcounts_num_below_maxshapes2.tex <==
26

==> stats/testcounts_num_below_maxshapes5.tex <==
26

==> stats/testcounts_num_below_maxshapesinfty.tex <==
26

==> tables/readstowrites.tex <==
\begin{tabular}{l | c}
\hline
benchmark&reads / writes\\
\hline
splay&1.4\\
bitwise-and&2.0\\
partial-sums&2.0\\
nsieve-bits&2.4\\
bits-in-byte&2.4\\
3bits-byte&2.4\\
nsieve&2.4\\
binary-trees&2.7\\
navier-stokes&2.9\\
nbody&3.4\\
v8-raytrace&4.4\\
fannkuch&4.5\\
earley-boyer&5.2\\
fasta&5.4\\
richards&5.5\\
3d-cube&8.3\\
3d-morph&15.8\\
deltablue&21.6\\
base64&27.4\\
3d-raytrace&37.6\\
v8-crypto&65.7\\
spectral-norm&179.6\\
crypto-sha1&225.7\\
crypto-md5&241.6\\
recursive&358.7\\
cordic&566.6\\
\hline
geo mean&11.7\\
\hline
\end{tabular}

